The Partially Observable Games We Play for Cyber Deception

Progressively intricate cyber infiltration mechanisms have made conventional means of defense, such as firewalls and malware detectors, incompetent. These sophisticated infiltration mechanisms can study the defender's behavior, identify security caveats, and modify their actions adaptively. To tackle these security challenges, cyber-infrastructures require active defense techniques that incorporate cyber deception, in which the defender (deceiver) implements a strategy to mislead the infiltrator. To this end, we use a two-player partially observable stochastic game (POSG) framework, wherein the deceiver has full observability over the states of the POSG, and the infiltrator has partial observability. Then, the deception problem is to compute a strategy for the deceiver that minimizes the expected cost of deception against all strategies of the infiltrator. We first show that the underlying problem is a robust mixed-integer linear program, which is intractable to solve in general. Towards a scalable approach, we compute optimal finite-memory strategies for the infiltrator by a reduction to a series of synthesis problems for parametric Markov decision processes. We use these infiltration strategies to find robust strategies for the deceiver using mixed-integer linear programming. We illustrate the performance of our technique on a POSG model for network security. Our experiments demonstrate that the proposed approach handles scenarios considerably larger than those of the state-of-the-art methods.

==> flowchart_deception.tex <==
%color scheme
%background 
\definecolor{bg}{HTML}{ddeedd}
\definecolor{comp}{HTML}{c2d4dd}
\definecolor{impl}{HTML}{b0aac0}
\centering
\begin{tikzpicture}[every node/.style={draw, text centered, shape=rectangle, rounded corners, text width=3.8cm, minimum height=1.5cm, inner sep=5pt}]
%\tikzstyle{outer}= [draw, text centered, shape=rectangle, text width=2cm, minimum height=1cm]
%\tikzstyle{inner}=[draw, text centered, shape=rectangle, rounded corners, text width=3.8cm, minimum height=1.1cm, inner sep=5pt]
\tikzset{
splitnode/.style={
       rectangle split,
       rectangle split parts=2,
       rectangle split part fill={comp,impl!50}
       }
}

\tikzset{
normalnode/.style={
	   fill=comp
       }
}



\tikzstyle{split}=[rectangle split,rectangle split parts=2]


\node[splitnode] (deceiver) {\textbf{Deceiver} \nodepart{second} Player~$1$ with Full Observability};

\node[splitnode, below=1.5cm of deceiver] (infiltrator) {\textbf{Infiltrator} \nodepart{second} Player~$2$ with Partial Observability};

\begin{scope}[on background layer]
	\node [fit = (current bounding box), inner sep = .5cm,  fill=bg] (posg) {\textbf{POSG -- Deception Game}};        
\end{scope}

\node[splitnode, right=2cm of deceiver] (pmdp) {\textbf{Infiltrator's Strategies} \nodepart{second} Parametric Markov Decision Process};

\node[splitnode, above=1.5cm of pmdp] (memory) {\textbf{Memory} \nodepart{second} Finite State Controller};

%
\node[splitnode, right=2cm of infiltrator] (mdp) {\textbf{Robust Deception Model} \nodepart{second} Markov Decision Process};

\node[splitnode, right=2cm of mdp] (strategy) {\textbf{Deceiver's Strategy} \nodepart{second} Optimal MDP Strategy};

\node[normalnode, above=2cm of strategy, minimum height=1cm] (spec) {\textbf{Deception/Infiltration Properties}};

	
%

%%arrows
\draw ([yshift=1.59cm] posg.east) edge[-latex', very thick] ([] pmdp.west);
\draw ([yshift=-1.59cm] posg.east) edge[-latex', very thick] ([] mdp.west);

\draw (pmdp) edge[-latex', very thick] (mdp);
\draw (mdp) edge[-latex', very thick] (strategy);

\draw (spec) edge[-latex', very thick, dashed] (pmdp);
\draw (spec) edge[-latex', very thick, dashed] (strategy);

\draw (memory) edge[-latex', very thick] (pmdp);
%\draw (pmdp) edge[-latex', very thick] (memory);


\end{tikzpicture}


==> preliminaries.tex <==
% !TeX spellcheck = en_GB

\section{Preliminaries - Collection of Definitions}
\label{sec:preliminaries}
\noindent 

Let $\Var=\{p_1,\ldots,p_n\}$ be a finite set of \emph{parameters} over the domain $\R$ and let $\poly[\Var]$ be the set of multivariate polynomials over $\Var$.
An \emph{instantiation} for $\Var$ is a function $u \colon \Var \to \R$.
Replacing each parameter $p$ in a polynomial $f \in \poly[\Var]$ by $u(p)$ yields $f[u] \in \R$; $f \neq 0$ holds if $f[u] \neq 0$ for some instantiation $u$.

%Decision problems can be considered as languages describing all positive instances. A language $L_1 \subseteq \{0,1\}^{*}$ is \emph{polynomial (many-one or Karp) reducible} to $L_2 \subseteq \{0,1\}^{*}$, written $L_1 \polred L_2$, if there exist a polynomial-time computable function $f\colon \{0,1\}^{*} \rightarrow \{0,1\}^{*}$ such that for all $w \in \{0,1\}^{*}$, $w \in L_1 \iff f(w) \in L_2$. Polynomial reductions are essential to define complexity classes, cf.~\cite{DBLP:books/daglib/0072413}.

\paragraph{Parametric Markov Decision Processes}
\label{ssec:prob_models}


%
The \emph{available actions} in $s\in\states$ are $\Act(s)=\{\act\in\Act\mid \exists s'\in\states: \probmdp(s,\act,s')\neq 0\}$.
We assume that pMDP $\mdp$ contains no deadlock states, \ie $\Act(s)\neq\emptyset$ for all $s\in\states$.
A \emph{path} of a pMDP $\mdp$ is an (in)finite sequence $\pi = s_0\xrightarrow{\act_0}s_1\xrightarrow{\act_1}\cdots$,
where $s_0=\sinit$, $s_i\in\states$, $\act_i\in\Act(s_i)$, and $\probmdp(s_i,\act_i,s_{i+1})\neq 0$ for all $i\in\N$.
For finite $\pi$, $\last{\pi}$ denotes the last state of $\pi$. 
The set of (in)finite paths of $\mdp$ is $\pathsfin^{\mdp}$ ($\pathset^{\mdp}$).
%
\begin{definition}[MDP]
  \label{def:mdp}
  A \emph{Markov decision process (MDP)} is a pMDP where $\probmdp \colon\states \times \Act \times \states \rightarrow [0,1] \subseteq \R$
  and  for all $s \in \states$ and $\act \in \Act(s)$ it holds that $\sum_{s'\in\states}\probmdp(s,\act,s') = 1$.
\end{definition}

A \emph{(parametric) discrete-time Markov chain} ((p)MC) is a (p)MDP with $|\Act(s)|=1$ for all $s\in\states$.
For a pMC $\dtmc$, we may omit the actions and use the notation $\pDtmcInit$ with a transition function $\probdtmc$
of the form $\probdtmc\colon\states\times\states\rightarrow \poly[\Var]$.
This is analogous for (non-parametric) MCs.

Applying an \emph{instantiation} $u\colon\Var\to\R$ to a pMDP or pMC $\mdp$, denoted $\mdp[u]$, replaces each polynomial
$f$ in $\mdp$ by $f[u]$. $\mdp[u]$ is also called the \emph{instantiation} of $\mdp$ at $u$.
Instantiation $u$ is \emph{well-defined} for $\mdp$ if the replacement yields probability distributions, \ie
if $\mdp[u]$ is an MDP or an MC, respectively.

%\paragraph{Strategies.}
To resolve the nondeterministic action choices in MDPs, so-called \emph{strategies} determine at each state a distribution over actions to take.
This decision may be based on the \emph{history} of the current path.
%
\begin{definition}[Strategy]
  \label{def:strategy}
  A \emph{strategy} $\sched$ for $\mdp$ is a function $\sched\colon \pathsfin^{\mdp}\to\Distr(\Act)$
  s.\,t.\ $\supp\bigl(\sched(\pi)\bigr) \subseteq \Act\bigl(\last{\pi}\bigr)$ for all $\pi\in \pathsfin^{\mdp}$.
  The set of all strategies of $\mdp$ is $\Sched^{\mdp}$.
\end{definition}
%
A strategy $\sched$ is \emph{memoryless} if $\last{\pi}=\last{\pi'}$ implies $\sched(\pi)=\sched(\pi')$ for all $\pi,\pi'\in\pathsfin^{\mdp}$.
It is \emph{deterministic} if $\sched(\pi)$ is a Dirac distribution for all $\pi\in\pathsfin^{\mdp}$.
A strategy that is not deterministic is \emph{randomised}.

A strategy~$\sigma$ for an MDP $\mdp$ resolves all nondeterministic choices, yielding an \emph{induced Markov chain} $\DTMCgnd$,
for which a \emph{probability measure} over the set of infinite paths is defined
 by a cylinder set construction~\cite{BK08}.

\begin{definition}[Induced Markov Chain]
  \label{def:induced_dtmc}
 For an MDP $\MdpInit$ and a strategy $\sched\in\Sched^{\mdp}$,  the MC induced by  $\mdp$ and $\sched$ is given by $\DTMCgnd = (\pathsfin^{\mdp},\sinit,\probdtmc^{\sched})$ where:
  \[
    \probdtmc^{\sched}(\pi,\pi') = \begin{cases}
        \probmdp(\last{\pi},\act,s')\cdot\sched(\pi)(\act) & \text{if $\pi' = \pi\act s'$,} \\
        0 & \text{otherwise.}
      \end{cases}
  \]
\end{definition}\nj{definition of induced MC may be omitted}



\paragraph{Partially Observable Markov Decision Processes}
\label{ssec:partial_obs}
%

\begin{definition}[POMDP]
  \label{def:pomdp}
  A \emph{partially observable MDP (POMDP)} is a tuple $\PomdpInit$, with $\MdpInit$ the \emph{underlying MDP of $\pomdp$}, $\ObsSym$ a finite set of observations and $\ObsFun\colon\states\rightarrow\ObsSym$ the \emph{observation function}.
\end{definition}
%
We require that states with the same observations have the same set of
enabled actions, \ie $\ObsFun(s)=\ObsFun(s')$ implies $\Act(s)=\Act(s')$ for all $s,s'\in\states$.
We define $\Act(z) = \Act(s)$ if $\ObsFun(s) = z$.
More general observation functions~\cite{RoyGT05,ShaniPK13} take the last action into account and provide a distribution
over $\ObsSym$. There is a transformation of the general case to the POMDP definition used here
that blows up the state space polynomially~\cite{ChatterjeeCGK16}.
%In Fig.~\ref{fig:pomdpfragment}, a fragment of the underlying MDP of a POMDP has two different observations,
%indicated by the state colouring.

We lift the observation function to paths: For
$\pi=s_0\xrightarrow{\act_0} s_1\xrightarrow{\act_1}\cdots s_n\in\pathsfin^{\mdp}$, the associated
\emph{observation sequence} is $\ObsFun(\pi)=\ObsFun(s_0)\xrightarrow{\act_0} \ObsFun(s_1)\xrightarrow{\act_1}\cdots\ObsFun(s_n)$.
Several paths in the underlying MDP may yield the same observation sequence.
Strategies have to take this restricted observability into account.
%
\begin{definition}
  \label{def:obsstrategy}
  An \emph{observation-based strategy} for a POMDP $\pomdp$ is a strategy
  $\osched$ for the underlying MDP $\mdp$
  such that $\osched(\pi)=\osched(\pi')$ for all $\pi,\pi'\in\pathsfin^{\mdp}$
  with $\ObsFun(\pi)=\ObsFun(\pi')$.
  $\oSched^\pomdp$ is the set of observation-based strategies for $\pomdp$.
\end{definition}
%
An observation-based strategy selects actions based on observations along a path and the past actions.
Applying the strategy to a POMDP yields an induced MC as in Def.~\ref{def:induced_dtmc}, resolving all nondeterminism and partial observability.
To represent observation-based strategies with finite memory, we one may use \emph{finite-state controllers} (FSCs).\nj{add references}
%A randomized observation-based strategy for a POMDP $\pomdp$ with (finite) $k$ memory is represented by an FSC $\fsc$ with $k$ memory nodes.
%If $k=1$, the FSC describes a \emph{memoryless strategy}.
%In the following, we refer to observation-based strategies as FSCs.
%
%\begin{figure}[tb]
%  \centering
%  \subfigure[POMDP $\pomdp$]{
%    \label{fig:pomdpfragment}
%    \scalebox{0.65}{
%      \input{pics/pomdp_fragment}
%    }
%  } \\
%  \subfigure[FSC $\fsc$]{
%    \label{fig:fsc_for_pomdp}
%    \scalebox{0.55}{
%      \input{pics/fsc_for_pomdp}
%    }
%  }
%  \subfigure[Induced MC $\pomdp^{\osched_\fsc}$]{
%    \label{fig:induced_mc_fsc_pomdp}
%    \scalebox{0.65}{
%      \input{pics/induced_pomdp_fsc}
%    }
%  }
%  \caption{(a)~The POMDP~$\pomdp$ has two observations $\ObsFun(s_1)=\ObsFun(s_3)=\obs_0$ (white)
%    and $\ObsFun(s_2)=\ObsFun(s_4)=\ObsFun(s_5)=\obs_1$ (red).
%    (b)~The associated (partial) FSC~$\fsc$ has two memory nodes.
%    (c)~The MC~$\pomdp^{\osched_\fsc}$ induced by $\pomdp$ and $\fsc$ has then $9$ states.
%  }
%  \label{fig:pomdp_and_fsc}
%\end{figure}
%
%\begin{definition}[FSC]
%  \label{def:fsc}
%  A \emph{finite-state controller (FSC)} for a POMDP $\pomdp$ is a tuple $\FSCinit$, where $N$ is a finite set of \emph{memory nodes},
%  $\ninit\in N$ is the \emph{initial memory node}, $\actionMap$ is the \emph{action mapping} $\actionMap\colon N\times\ObsSym\rightarrow\Distr(\Act)$,
%  and $\nodeTransition$ is the \emph{memory update} $\nodeTransition\colon N\times\ObsSym\times\Act\rightarrow \Distr(N)$.
%  The set $\FSCs[k]{\pomdp}$ denotes the set of FSCs with $k$ memory nodes, called \emph{$k$-FSC}s.
%  Let $\osched_\fsc\in\oSched^\pomdp$ denote the observation-based strategy represented by $\fsc$.
%\end{definition}
%%
%From a node $n$ and the observation $\obs$ in the current state of the POMDP, the next action $\act$ is
%chosen from $\Act(\obs)$ randomly as given by $\actionMap(n, \obs)$. Then, the successor node of the FSC is determined randomly as
%described by $\nodeTransition(n, \obs, \act)$.

%\begin{example}
%  \label{ex:constant_induced_mc}
%  Fig.~\ref{fig:fsc_for_pomdp} shows an excerpt of an FSC $\fsc$
%  with two memory nodes.
%  From node $n_1$, the action mapping distinguishes observations $\obs_0$ and $\obs_1$.
%  The solid dots indicate a probability distribution from $\Distr(\Act)$.
%  For readability, all distributions are uniform and we omit the action mapping for node $n_2$.
%
%  Now recall the POMDP $\pomdp$ from Fig.~\ref{fig:pomdpfragment}.
%  The induced MC~$\pomdp^{\osched_\fsc}$ is shown in Fig.~\ref{fig:induced_mc_fsc_pomdp}.
%  Assume $\pomdp$ is in state $s_1$ and $\fsc$ in node $n_1$.
%  Based on the observation $\obs_0\colonequals\ObsFun(s_1)$, $\osched_\fsc$ chooses action $\act_1$ with probability $\nodeTransition(n_1,\obs_0)(\act_1)=0.5$  leading to the probabilistic branching in the POMDP.
%  With probability $0.6$, $\pomdp$ evolves to state $s_2$.
%  Next, the FSC $\fsc$ updates its memory node; with probability $\nodeTransition(n_1, \obs_0, \act_1)(n_1)=0.5$, $\fsc$ stays in $n_1$.
%  The corresponding transition from $\langle s_1,n_1\rangle$ to $\langle s_2,n_1\rangle$
%  in  $\pomdp^{\osched_\fsc}$ has probability $0.5\cdot 0.6\cdot 0.5=0.15$.
%\end{example}


\subsection{Specifications}
\label{ssec:spec}

%For a POSG $\posg$, a set $G\subseteq\states$ of \emph{goal states}, a set $B\subseteq\states$ of \emph{bad states}, and a \emph{threshold} $\lambda \in [0,1]$, we consider \emph{quantitative reach-avoid specifications}
%$\varphi=\p_{> \lambda} (\neg B\,\Until\,G)$. The specification $\varphi$ is satisfied for a
%strategy $\osched\in\oSched^\pomdp$ if the probability $\pr^{\pomdp^\osched}(\neg B\,\Until\,G)$ of reaching a goal state in $\pomdp^\osched$
%without entering a bad state in between exceeds $\lambda$, denoted by $\pomdp^\osched\models\varphi$.
For a POSG $\posg$, a set $B\subseteq\states$ of \emph{bad states}, and a \emph{threshold} $\lambda \in [0,1]$, we consider \emph{quantitative reachability specifications}
$\varphi=\p_{\leq \lambda} (\finally B)$. The specification $\varphi$ is satisfied for a
strategy $\osched\in\oSched^\pomdp$ if the probability $\pr^{\pomdp^\osched}(\finally B)$ of reaching a bad state in $\pomdp^\osched$ is at most $\lambda$, denoted by $\pomdp^\osched\models\varphi$.
Vice versa, a strategy $\sched'\in\oSched^\pomdp$ refutes the specification, denoted by $\pomdp^\osched\not\models\varphi$, if $\pr^{\pomdp^\osched}(\finally B)>\lambda$.


The task is to compute such a strategy provided that one exists. 
For an MDP $\mdp$, there is a memoryless deterministic strategy inducing the maximal (or minimal) probability $\pr_{\max}^\mdp(\neg B\,\Until\,G)$~\cite{Condon92}.
For a POMDP $\pomdp$, however, observation-based strategies with infinite memory as in Def.~\ref{def:obsstrategy} are necessary~\cite{Ross83}.
The problem of proving the satisfaction of $\varphi$ is therefore undecidable~\cite{ChatterjeeCT16}.
%In our experiments, we also use \emph{undiscounted expected reachability reward properties}~\cite{BK08}.
